Regression and Classification for Direction-of-Arrival Estimation with Convolutional Recurrent Neural Networks

We present a novel learning-based approach to estimate the direction-of-arrival (DOA) of a sound source using a convolutional recurrent neural network (CRNN) trained via regression on synthetic data and Cartesian labels. We also describe an improved method to generate synthetic data to train the neural network using state-of-the-art sound propagation algorithms that model specular as well as diffuse reflections of sound. We compare our model against three other CRNNs trained using different formulations of the same problem: classification on categorical labels, and regression on spherical coordinate labels. In practice, our model achieves up to 43% decrease in angular error over prior methods. The use of diffuse reflection results in 34% and 41% reduction in angular prediction errors on LOCATA and SOFA datasets, respectively, over prior methods based on image-source methods. Our method results in an additional 3% error reduction over prior schemes that use classification based networks, and we use 36% fewer network parameters.

==> from_report/1_introduction.tex <==
\section{Introduction}
Estimating the direction of arrival (DOA) of audio sources has been studied for many years in the signal processing community. In this problem, the goal is to predict the azimuth and elevation angles of the sound source relative to the microphone, from a sound clip recorded in spatial audio format. There are several problems within this domain that vary in their degrees of complexity. One of the simpler problems is the estimation of direction-of-arrival (DOA) on the horizontal plane. More complex problems include DOA estimation in three-dimensional space or identification of both direction and distance of an audio source. The most complex problems involve achieving the aforementioned goals in noisy or reverberant environments.

The general architecture of a DOA estimation system is described in Figure ~\ref{fig:system}. Intuitively, there are several dimensions to be explored when designing a system for DOA estimation, including feature representations, network architecture, and output representation. The choice of each variable has an observable effect on the performance of the trained model.

\begin{figure}[htbp]
\centering \includegraphics[width=\linewidth]{system}
 \caption{General architecture of a DOA estimation system. Raw audio signal is featurized as a vector x, and the corresponding DOA is encoded as a vector y, which the model can predict given x. Model is trained to map features X to targets Y by gradient descent. During inference, predictions are decoded to determine the DOA.}
\label{fig:system}
\end{figure}

Existing research suggests that deep, sequential architecture may be better suited to DOA estimation. One paper suggests that classification outperforms regression for DOA estimation, though results were not documented. Moreover, the representation of DOA as a cartesian coordinate is more natural and less prone to errors, so there is an incentive to explore and document results for the regression formulation of our problem.

In this project, we explored the application of neural networks to DOA estimation of speech in the presence of noise and reverberation. The objective of our research is to model the dependence of accuracy on the variables in the DOA estimation system, for a single static source. In the short semester we have, we focused on output representation, assuming a modern neural network approach, working our way from the state-of-the-art model to more general cases. We experimented with different architectures and found that the regression formulation yields higher accuracy. We were able to train a model that outperforms the state-of-the-art on our dataset of simulated SRIRs.

We used a state-of-the-art acoustic simulator to build our dataset, which consists of speech with DOAs uniformly distributed around an Ambisonic (see Section~\ref{sec:ambisonic}) microphone array. Features extracted from the channels of the speech recording form the input to our networks. We compare output formulations (regression vs. classification) as well as architectures (convolutional neural network (CNN) vs. convolutional \textit{recurrent} neural network (CRNN)). We find that a CRNN regressor outperforms other models.

==> from_report/2_related_work.tex <==
\section{Related Work}

\subsection{Overview}
We begin with an overview of existing works. One classic approach to DOA estimation is to first determine the time delay of arrival (TDOA) between microphone array channels, which can be estimated by generalized cross correlation~\cite{knapp1976gcc} or by least squares~\cite{huang2001ls}. With TDOA and knowledge of the array layout, the DOA follows directly. Another approach is to use the signal subspace as in the MUSIC algorithm~\cite{schmidt1986music}. With some restrictions on operating conditions, these techniques can be very effective. However, they do not perform well in highly reverberant and noisy environments, or when the placement of signal sources is free to be arbitrary~\cite{dibiase2001robust}. More recently, researchers have applied modern machine learning techniques to speech DOA estimation with the goal of improving performance in noisy, realistic environments. In this paper, we focus on neural network approaches. In particular, we primarily investigate approaches along three dimensions: input features, network architecture, and output representation.
\subsection{Classification}
Xiao et al.~\cite{xiao2015learning} feed features from generalized cross correlation vectors of microphone array input to a multilayer perceptron neural network. They show superior performance over the classic least square method~\cite{huang2001ls} in both simulated and real rooms of varying sizes. Perotin et al.~\cite{perotin2018crnn} calculate acoustic intensity vectors from a first-order Ambisonics representation of audio. This representation serves as input to a CRNN, which yields more accurate predictions than a baseline approach using independent component analysis. Adavanne et al.~\cite{adavanne2017crrnmulti} also use CRNNs and apply it to the problem of identifying DOA when there are overlapping sound sources. Each of these approaches frames DOA estimation as a classification problem. A discrete number of possible DOAs (either in one angular dimension~\cite{xiao2015learning} or two~\cite{perotin2018crnn,adavanne2017crrnmulti}) is evenly distributed in space for training and test data. The outputs of the predictive models are probabilities that each of the possible DOAs is correct.
\subsection{Regression}
Xiao et al. claim that they tested regression formulation of DOA estimation and saw worse performance than the classification formulation for their network. However, they do not present results from the experiments that substantiate this claim. Perotin et al. use this as a reason to avoid developing and testing a regression version of their CRNN. The lack of results for regression in these instances was the primary motivation for exploring regression in this project.

Two very recent papers have reported the results of applying neural network regression to DOA estimation. Vera-Diaz et al. use CNN regression to estimate the cartesian coordinates of a sound source in three-dimensional space~\cite{veradiaz2018CNN}. Adavanne et al. publish a follow-up to their 2017 paper where they use CRNN regression instead of classification~\cite{adavanne2018crrnreg}. They find higher error for DOA estimates with regression than with classification, which is consistent with the claims of Xiao et al. but inconsistent with the findings of this paper. Some differences to highlight between our work and their work are 1) they do not use Ambisonic audio as input to their network and 2) they add the additional complication of overlapping sound sources.

\begin{table}[htbp]
\label{tab:other_models}
\caption{List of existing models.}
\centering
\begin{tabular}{lllllc}
\toprule
 Approach & Input features & Output format & Formulation & Network \\\hline
 Vesperini et al. & GCC & x,y & Reg & MLP \\
 Vesperini et al. & GCC & x,y & Reg & CNN \\
 Ferguson et al. & GCC,cepstrogram & azi,dist & Reg & CNN  \\
 Vera Diaz et al. & GCC & x,y & Reg & CNN \\
 Adavanne et al. & Phase and magnitude spectrum & azi,ele & Class & CRNN \\
 Adavanne et al. & STFT & azi,ele & Class & CRNN \\
 Xiao et al. & GCC & azi,ele & Class & MLP  \\
 Perotin et al. & STFT & azi,ele & Class & CRNN  \\
 \bottomrule
  \end{tabular}
\end{table}

\subsection{Comparison}

The state of the art model is a CRNN trained for the classification problem. We started with this architecture to perform our evaluation on classification and regression formulations. However, since the architecture is variable, we also experimented with the CNN, which has also been shown to perform well for some classification and regression tasks.


==> from_report/3_background.tex <==
\section{Background}
\subsection{First Order Ambisonics}
\label{sec:ambisonic}
In order to analyze spatial information from sound recordings, at least two microphones with known relative positions must be used. In practice, various stereo recording formats including binaural, 5.1-channel, 7.1-channel, etc. have been applied to spatial audio related systems. The Ambisonics format decomposes a soundfield using spherical harmonic function basis~\cite{gerzon1973periphony}. Compared with its alternatives, Ambisonics has the advantage of hardware independence - it does not encode speaker specifications into the recording, and can be reproduced using any spatial sound playback devices. This property makes it ideal for machine learning approaches, because the trained system does not need to be adjusted or re-trained for integration with an Ambisonic microphone different from the one used to produce the training data, which provides great hardware compatibility.

In theory, Ambisonics format that has an infinite number of basis can reproduce the recorded soundfield with no error. But we use the first order ambisonics (FOA) which has the first four basis/channels as an approximation. The FOA channels are denoted by $W, X, Y, Z$, where $W$ channel contains the zeroth-order coefficients that represent the omnidirectional signal intensity, and $X, Y, Z$ channels contain the first-order coefficients that encode direction modulated information. For a plane wave with azimuth $\theta$ and elevation $\phi$ creating a sound pressure $p$, the complex FOA components are:
\begin{gather}
\begin{bmatrix}
W(t,f) \\
X(t,f) \\
Y(t,f) \\
Z(t,f)
\end{bmatrix}
=
\begin{bmatrix}
1 \\
\sqrt{3}cos\theta cos\phi\\
\sqrt{3}sin\theta cos\phi \\
\sqrt{3}sin\phi
\end{bmatrix}
p(t,f),
\label{eq:foa}
\end{gather}
where $t$ and $f$ are time and frequency bins.

\subsection{Sound Propagation}
\label{sec:sound_propagation}
Sound propagation methods compute the reflection and diffraction paths from the sound sources to a listener in the virtual environment. Prior algorithms for sound propagation can be classified into two categories: geometric techniques and wave-based techniques. The nature of sound propagation can be explained using the wave equation:
\begin{equation}
\label{eq:waveequation}
\frac{\partial^2}{\partial t^2}P(\boldx,t)-c^2P(\boldx,t)=f(\boldx,t),
\end{equation}
where $c$ is the speed of sound in a homogeneous medium, which we assume to be $343m/s$, and $f(\boldx,t)$ is the forcing term at location $\boldx$ at time $t$. Wave-based sound propagation methods directly solve the wave equation for sound propagation (see Equation~\ref{eq:waveequation}). These methods are based on Finite Element Methods (FEM), Boundary Element Methods (BEM), finite-difference time domain (FDTD) approaches~\cite{sakamoto2006numerical} and Adaptive Rectangular Decomposition (ARD) methods~\cite{raghuvanshi2009efficient}. Wave-based techniques are accurate, but are only practical for low frequencies and small scenes. Geometric methods work on the underlying assumption of sound wave propagating in the form of a ray, where the wavelength of the sound is smaller than the size of the obstacles in the environment~\mbox{\cite{funkhouser2003survey}}. These methods include image source methods \mbox{\cite{allen1979image}}, ray tracing methods \mbox{\cite{vorlander1989,schissler2016interactive,schissler2016adaptive,schissler2014high}}, and beam or frustum tracing methods \mbox{\cite{funkhouser1998beam,chandak2008ad}}. They are mostly accurate for higher frequencies and can be used for interactive applications.

In speech/audio related training, the common practice is to use naive image source methods to generate synthetic impulse responses and use them to augment the training data~\cite{ko2017study}. However, image source methods do not model sound scattering, which is an important phenomenon in acoustic environments. This means no late reverberation is modeled during training. We utilize the state-of-the-art geometric sound renderer~\cite{schissler2014high} to generate our synthetic data, which will behave more like real sound recordings, compared with image source methods.

==> from_report/4_method.tex <==
\section{Method}

\subsection{Input Feature}
\label{sec:feature}
We follow the approach in~\cite{perotin2018crnn} to construct our input feature from raw FOA audio. The active and reactive intensity vectors are computed as:
\begin{gather}
\boldI_a(t,f)=
\begin{bmatrix}
\mathcal{R}\{W(t,f)*X(t,f)\} \\
\mathcal{R}\{W(t,f)*Y(t,f)\} \\
\mathcal{R}\{W(t,f)*Z(t,f)\}
\end{bmatrix}
,
\boldI_r(t,f)=
\begin{bmatrix}
\mathcal{I}\{W(t,f)*X(t,f)\} \\
\mathcal{I}\{W(t,f)*Y(t,f)\} \\
\mathcal{I}\{W(t,f)*Z(t,f)\}
\end{bmatrix},
\label{eq:intensity_vec}
\end{gather}
where $\mathcal{R}\{\cdot\}$ and $\mathcal{I}\{\cdot\}$ extract the real and imaginary components of a complex signal respectively. Both feature vectors are scaled as:
\begin{equation}
\label{eq:waveequation}
\frac{1}{|W(t,f)|^2+\frac{1}{3}(|X(t,f)|^2+|Y(t,f)|^2+|Z(t,f)|^2)}
\begin{bmatrix}
\boldI_a(t,f) \\
\boldI_r(t,f)
\end{bmatrix},
\end{equation}
to have a uniform range, which is beneficial for deep neural network training.

\subsection{Output Formulation}

The classification formulation of DOA estimation requires the discretization of the unit sphere into some number of possible output directions. We approximate a uniform distribution of output classes using a heuristic algorithm employed by Perotin et al.~\cite{perotin2018crnn}. This algorithm takes, as input, a desired angular resolution of the mesh of output directions and generates the set of DOA class directions. For our classifiers, we specify an angular resolution of 10 $\degree$, which results in 405 direction classes.

Each training DOA label is assigned to the direction class that it is has the smallest angular difference from. We use this labeling to train a classifier that outputs a softmax vector of the direction class. We choose cross-entropy loss as our training loss function.

For the regression formulation, the output of our networks is the three-dimensional Cartesian coordinates representing the estimated DOA. Training DOA labels are three-dimensional Cartesian coordinates that lie on the unit sphere. We choose mean-squared error to represent our regression loss. Note that the network output is not constrained to lie on the unit sphere. As a result, a hypothetical output that is a large scalar multiple of the DOA label will result in a large loss, despite the perfect alignment of the output vector with the label. However, we see in our results that this concern does not appear to constrain the performance of trained regression models.

Requisite for the comparison between models with different output formulations is a common metric. For this metric, we consider the angular error between estimated and actual DOAs.

\subsection{Network Architecture}

The CNN and CRNN that we trained for our experiments were implemented using the PyTorch framework with the Adam optimizer~\cite{adam}. As described in Section~\ref{sec:feature}, the inputs to these networks are active and reactive intensity vectors. The dimensionality of the input is therefore 6x25x513, corresponding to 6 intensity vectors, 25 frames, and 513 frequency bins.

The CRNN network architecture is shown in Figure~\ref{fig:architecture}. There are three convolutional layers, each layer consisting of two-dimensional convolution, batch normalization, a rectified linear unit (ReLU), and max pooling. The outputs of each or the three layers are 64x25x64, 64x25x8, and 64x25x2, respectively. The last layer's output is flattened into a 128-dimensional vector for each of the 25 frames. Each frame's vector is fed into a two-layer bi-directional LSTM, and the output of the LSTM for each frame is fed through two fully-connected linear layers. This yields a DOA estimate for each frame. As described in the previous section, this output will take the form of three-dimensional Cartesian coordinates for the regression formulation and a 405-dimensional softmax output for the classification formulation. During training, loss is computed separately for each frame for the purpose of backpropagation. During evaluation, the DOA estimate is taken to be the average of all estimates across frames.

The CNN network is identical to the CRNN except that the Bi-LSTM layer is removed and the output of the last convolutional layer is directly connected to the fully-connected layers.

\begin{figure}[htbp]
\centering \includegraphics[width=\linewidth]{architecture}
 \caption{Our network architecture, output format of the network can be switched in the output layer for regression or classification formulation.}
\label{fig:architecture} 
\end{figure}


==> from_report/5_experiment.tex <==
\section{Experiment}
\subsection{Data Preparation}
We generated 42000 rectangular room configurations with dimensions uniformly and independently sampled between $2.5m\times 2.5m\times 2m$ and $10m\times 10m\times 3m$. Under each room configuration, we randomly populate three paired source-listener locations, both at least $0.5m$ away from walls. Our data pre-processing pipeline is shown in Figure~\ref{fig:pipeline}. Geometric sound propagation is performed on each source-listener pair to generate its SRIR. Then we convolve the SRIR with a one-second clean speech from the Libri ASR corpus~\cite{panayotov2015librispeech} to generate realistic reverberant speech recordings in FOA format. A short time fourier transform (STFT) is used to convert speech wavforms to spectrogram, and the features are extracted according to Section~\ref{sec:feature}. The training is based on reverberant speech. In total, we have 126000 labeled data samples.
\begin{figure}[htbp]
\centering 
\includegraphics[width=\linewidth]{pipeline}
 \caption{Our data pre-processing pipeline. STFT was performed on 1024 points with $50\%$ overlapping, and the first 25 frames were used. Each sample had a dimension of 6 channels, 25 frames and 513 frequency bins.}
\label{fig:pipeline} 
\end{figure}

\subsection{Training Schedule}
We employed a 9:1 train-validation split of our dataset. All training was done on four TITAN X (Pascal) graphical units simultaneously. Hyperparameters including batchsize, learning rate were optimized using Bayesian search~\cite{snoek2012practical}. We tried both Adam and SGD optimizers, with and without dropout, and early stop with a 3-epoch patience, 30 epoches maximum, given that an epoch takes from 30 minutes to an hour. To maintain maximum consistency of our comparisons, the implementation of our CNN and CRNN networks share the same convolutional part, while classification and regression networks only differ in input and output layers.


\subsection{Metrics}
While our models are trained using different loss functions, we evaluate them under the same metrics. One intuitive metric is to measure the percentage of predictions that lie within some error tolerance. We decide to use the same error thresholds as in~\cite{perotin2018crnn}: $5\degree, 10\degree$, and $15\degree$. The prediction from the classification model is first mapped to its corresponding directional vector before calculating the angular distance.

We define four angular error metrics which measure the performance of our predictor for four different cases. The error metric takes arguments $(\hat{y},y)$ and outputs a percentage. Given any discretization of the output space into classes, we can map the vector of any given angle to the vector of the closest class (C), or keep the raw vector (X). Both operations can be applied to the angular prediction, and to the target vector. We label the metrics CC,CX,XC,XX for simplicity. The purpose of each metric is described below.
\begin{itemize}
    \item CC: Decode the predicted DOA, snap it to the closest class, and snap the target to class.
    \item CX: Decode the predicted DOA, snap it to the closest class, and leave the target as a raw vector.
    \item XC: Decode the predicted DOA, leave it as a raw vector, and snap the target to class.
    \item XX: Decode the predicted DOA, leave it as a raw vector, and leave the target as a raw vector.
\end{itemize}

Each metric gives us a proportion of the test examples that are correctly classified within a given set of thresholds, after mapping the predictions and targets according to the corresponding operations. There are several interesting scenarios that can be uncovered by comparing the predictors with these metrics. The superior model under XX can be interpreted as the model that should attain superior accuracy in a realistic scenario. Comparing models under CC allows us to put the classifier and regressor on the same playing field, so that we can compare the ability of SGD to fit the dataset under the classification and regression formulations, compensating for the discretized output space of the classifier; if the regressor outperforms the classifier under CC, it suggests that the regression formulation can solve for a model that, if its output is passed through a classification function, will still outperform the classifier trained via gradient descent on cross-entropy loss.


==> from_report/6_result.tex <==
\section{Results and Analysis}
We highlight results for all tests we’ve run in Table~\ref{tab:results}. We notice that in our tests, regression models outperform classification models; while CRNN yields better results than CNN under same formulations. Having higher grid resolution did not help achieve better numbers from limited number of tests. Although our final number looks more promising than the 2018 paper, we cannot safely draw a conclusion yet. Because the test dataset is different for~\cite{perotin2018crnn} and the authors couldn’t share the data for now.

\begin{table}[htbp]
\caption{Training results on different models. The best results are shown in bold. Note that we cannot make comparisons on the real data used by Perotin et al.~\cite{perotin2018crnn} because it was made private.}
\label{tab:results}
\centering
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Angular Error}   & \multicolumn{3}{c}{Simulated SRIR}  & \multicolumn{3}{c}{Real SRIR}       \\\cline{2-4}\cline{5-7}
       & $<5\degree$ & $<10\degree$ & $<15\degree$ & $<5\degree$ & $<10\degree$ & $<15\degree$ \\\hline
Perotin et al.~\cite{perotin2018crnn}      & 51.6$\%$        & 91.1$\%$         & 95.2$\%$         & 28.6$\%$        & 70.2$\%$         & 89.6$\%$         \\
CNN Classification  & 10.5$\%$        & 22.0$\%$         & 40.6$\%$         & \multicolumn{3}{c}{\multirow{4}{*}{Data inaccessible}}                     \\
CRNN Classification & 23.8$\%$        & 46.3$\%$         & 73.8$\%$         & \multicolumn{3}{l}{}                \\
CNN Regression      & 44.3$\%$        & 82.5$\%$         & 94.1$\%$         & \multicolumn{3}{l}{}                \\
CRNN Regression     & \textbf{90.6$\%$}        & \textbf{99.1$\%$}         & \textbf{99.5$\%$}        & \multicolumn{3}{l}{}    
\\\bottomrule
\end{tabular}
\end{table}

We also show the loss curve for our best models from hyperparameter search in Figure~\ref{fig:loss_curves}. One interesting observation was that small batches (e.g. 32 and 64) almost always outperform larger batches despite the large loss perturbations during training. This aligns with the intuition that small batches may add more randomness and prevent the training process from stopping at a local minimum too early.

\begin{figure}[htbp]
\centering 
% \includegraphics[width=\linewidth]{placeholder_flat}
    \subfigure[CNN Regression]{
        \includegraphics[width=0.48\linewidth]{figures/loss_cnn_reg.png}
    }
    \subfigure[CNN Classification]{
        \includegraphics[width=0.48\linewidth]{figures/loss_cnn_class.png}
    }
    \subfigure[CRNN Regression]{
        \includegraphics[width=0.48\linewidth]{figures/loss_crnn_reg.png}
    }
    \subfigure[CRNN Classification]{
        \includegraphics[width=0.48\linewidth]{figures/loss_crnn_class.png}
    }
 \caption{Loss curves during training and validation.}
\label{fig:loss_curves} 
\end{figure}

To test the robustness of our model under input noise, we added gaussian white noise to the validation samples and evaluate our best CRNN regression model on it. Noise was added according to signal to noise ratios of $30$dB, $20$dB, $10$dB and $0$dB. We have plotted several metrics for varying SNR levels. The angular accuracy for each threshold tends to decrease significantly as more noise is added to the signal. Comparing the SNR curves for the classifier and the regressor, we observe that our regression model is more robust to noise than the state-of-the-art model trained on our dataset of simulated SRIRs.

\begin{figure}[htbp]
\centering 
\includegraphics[width=0.8\linewidth]{figures/cccx.png}
    % \subfigure[$5\degree$ Threshold]{
    %     \includegraphics[width=0.31\linewidth]{figures/placeholder_flat.pdf}
    % }
    % \subfigure[$10\degree$ Threshold]{
    %     \includegraphics[width=0.31\linewidth]{figures/placeholder_flat.pdf}
    % }
    % \subfigure[$15\degree$ Threshold]{
    %     \includegraphics[width=0.31\linewidth]{figures/placeholder_flat.pdf}
    % }
    
 \caption{Error curves under different level or noise.}
\label{fig:snrerror} 
\end{figure}

==> from_report/7_discussion.tex <==
\section{Discussion and Future Work}

There are several interesting takeaways from the results of our experiments. First, we see that the CRNN outperforms the CNN for both classification and regression. This does not come as a huge surprise to us, as we predicted that a network capable of capturing the sequential nature of audio input would be more effective at predicting DOAs.

Second, we see that the regression formulations outperform classification formulations. This result is surprising because it is contrary to literature suggesting that regression for DOA estimation underperforms classification~\cite{xiao2015learning}~\cite{adavanne2018crrnreg}. It's not clear what the discrepancy is here, but the best way to start narrowing it down would be to exactly re-implement the network architectures documented in the cited papers and run our experiments on them.

To supplement our results on simulated recordings, we plan to set up a physical experiment. This will require procuring the necessary hardware for recording and production of speech. We hope to see results that are consistent with what the simulated experimental setup has yielded.


\begin{figure}[htbp]
\centering 
\includegraphics[width=\linewidth]{demo}
\caption{A screenshot of our demo/visualization system that can let us visually interpret error sources under different room settings.}
\label{fig:demo} 
\end{figure}
